Online Learning and Distributed Control for Residential Demand Response

This paper studies the automated control method for regulating air conditioner (AC) loads in incentive-based residential demand response (DR). The critical challenge is that the customer responses to load adjustment are uncertain and unknown in practice. In this paper, we formulate the AC control problem in a DR event as a multi-period stochastic optimization that integrates the indoor thermal dynamics and customer opt-out status transition. Specifically, machine learning techniques including Gaussian process and logistic regression are employed to learn the unknown thermal dynamics model and customer opt-out behavior model, respectively. We consider two typical DR objectives for AC load control: 1) minimizing the total demand, 2) closely tracking a regulated power trajectory. Based on the Thompson sampling framework, we propose an online DR control algorithm to learn customer behaviors and make real-time AC control schemes. This algorithm considers the influence of various environmental factors on customer behaviors and is implemented in a distributed fashion to preserve the privacy of customers. Numerical simulations demonstrate the control optimality and learning efficiency of the proposed algorithm.

==> bio.tex <==

% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)

\vskip -4pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{CX}}]{Xin Chen}
received his double B.S. degrees in engineering physics and economics from Tsinghua University, Beijing, China in 2015, and the master degree in electrical engineering from Tsinghua University, Beijing, China in 2017. He is 
currently pursuing the Ph.D. degree in electrical engineering at Harvard University, USA. 
He received the Best Conference Paper Award in IEEE PES General Meeting 2016, and he was a Best Student Paper Award Finalist in the IEEE Conference on Control Technology and Applications (CCTA) 2018. His research interests focus on 
distributed optimization, control, and learning of networked systems, with emphasis on power and energy systems.
\end{IEEEbiography}


\vskip 0pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{yingying}}]{Yingying Li}
 ...
\end{IEEEbiography}

\vskip 0pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Jun}}]{Jun Shimada}
is the founder of ThinkEco, a start up focused on residential demand response.  He received his PhD from Harvard University in Chemical Physics, and did postdoctoral research in theoretical biophysics at Columbia University and NYU.  Prior to ThinkEco, he was a founding team member of Vitae Pharmaceuticals, where he was the lead scientist behind its computational drug discovery platform.  His work has led to awards from various organizations, including the Alliance to Save Energy, International CES, and Powergrid International.  A serial entrepreneur, he is always looking to apply rigorous theoretical concepts to the next big idea.
\end{IEEEbiography}


\vskip 0pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{lina}}]{Na Li}
 is a Gordon McKay professor in Electrical Engineering and Applied
Mathematics at Harvard University. She received her Bachelor degree in
Mathematics from Zhejiang University in 2007 and Ph.D. degree in Control
and Dynamical systems from California Institute of Technology in 2013. She
was a postdoctoral associate at Massachusetts Institute of Technology 2013-
2014. Her research lies in control, learning, and optimization of networked
systems, including theory development, algorithm design, and applications
to real-world cyber-physical societal system in particular power systems. She
received NSF career award (2016), AFSOR Young Investigator Award (2017),
ONR Young Investigator Award(2019), Donald P. Eckman Award (2019),
McDonald Mentoring Award (2020), along with some other awards.
\end{IEEEbiography}






%\begin{IEEEbiographynophoto}{Jane Doe}
%Biography text here.
%\end{IEEEbiographynophoto}
